Why a Particle Physicist is Interested in DNA Branch Migration

We describe an explicitly discrete model of the process of DNA branch migration. The model matches the existing data well, but we find that branch migration along long strands of DNA ($N \simge 40$~bp) is also well modeled by continuum diffusion. The discrete model is still useful for guiding future experiments.

==> TXSdcol.tex <==
%% file: TXSdcol.tex  (TeXsis version 2.17)
%  $Revision: 17.1 $  :  $Date: 1995/02/23 23:44:02 $  :  $Author: myers $
%======================================================================*
% Double Column Output Routines:
%
% These macros let you create double column output, with balancing
% of partially filled columns, and with top, bottom, and footnote
% insertions in the columns or across the width of the page.
%
% To set up for double column output on a page of a given <width> and
% <height> and with columns of width <c-width> put the following at the
% beginning of your document:
%
%       \hsize=<width>  \vsize=<height>
%       \SetDoubleColumns{<c-width>}
%
% Note that this re-defines TeX's \output routine.  It does not actually 
% put you in double column mode.  To do that, say \doublecolumns.  To
% switch back to single column output say \enddoublecolumns (or the
% synonym \singlecolumn).   Partially filled columns will be balanced
% to the best of TeX's abilities.
%
% The usual insertions of TeX and TeXsis (\topinsert, \midinsert,
% \pageinsert, \heavyinsert and \bottominsert) put insertions into the
% current column.  To force an insertion into a particular column, say
% \forceleft or \forceright INSIDE the insertion material.  
%
% Wide insertions across the width of both columns can be made with
% \widetopinsert, \widepageinsert, or \widebottominsert.  
%
% Long equations which need to span both columns should be enclosed
% between \longequation (before the first "$$") and \endlongequation
% (after trailing "$$").  Rules to guide the eye are put at the bottom
% of the left column above the equation and above the right column below
% the equation (as is done in Physical Review).  You can change this.
%
% Footnotes created with \footnote or \vfootnote will be placed at the
% bottom of the current column.  You can place a footnote across the
% bottom of both columns with \widefootnote or \widevfootnote.
%
% You can always force a skip to the next column with \newcolumn.
% To skip to a completely new page use \vfill\eject, as usual.
%
% In single column mode all of these macros either behave as their
% single-column counterparts or do nothing, as appropriate, so that
% your document comes out looking right in single column mode.
%
% WARNING!  Formatting double column documents is inherently more
% difficult than regular typesetting.  Here are some helpful hints:
%   (1) Since double columns are narrow, the normal TeX spacing produces 
% many overfull \hbox's. To avoid this, the interword skip \spaceskip is
% changed to \doublecolskip=.3333em plus .3333em minus .1em
% More uniform spacing can be obtained by changing \doublecolskip.
%   (2) The value of \vbadness and \hbadness are doubled in double
% column mode, but you may want to increase them further to avoid
% complaints of overfull boxes.  But don't increase these too much.
%   (3) To balance columns it is essential to have some stretch in the
% column.  Using \parskip=\smallskipamount helps, or try adding a little
% stretch to the \baselineskip with: \advance\baselineskip by 0pt plus 0.5pt
%
% This version of these macros is a complete re-write of the TeXsis
% double column macros previous to version 2.16.  Some of the methods
% used here are adapted from The TeXBook, pg 417, and The TUGboat, Vol
% 6, pg 29.  See the file TXSdcol.doc for further documentation.
%
% Dependencies:  none -- this file can be used as it is with plain.tex,
%
% This file is a part ot TeXsis, a set of TeX macros for Physicists
% (C) copyright 1994 by Eric Myers and Frank Paige.
%======================================================================*
\message{- Double column format.}

\catcode`@=11                                   % make @ a letter for this file

\newdimen\colwidth                              % width of column
\newdimen\pagewidth                             % total width of page
\newdimen\pageheight                            % total height of page
\newdimen\rulewd          \rulewd=.5pt          % col. rule height
\newdimen\colmaxdepth     \colmaxdepth=4pt      % max. split depth
                                                
\newdimen\@bigColHeight         % height of both columns together
\newdimen\@saveSplitmax         % to save \splitmaxdepth
\newdimen\@saveVsize            % to save \vsize
\newskip\s@veskip               % to save \spaceskip
\newskip\doublecolskip          % new \spaceskip
\doublecolskip=.3333em plus .3333em minus .1em  % with more stretch

\newdimen\@leftpluscenter       % how far to move over for rule

\newbox\partialpage             % save single column partial page here

\newif\ifleftc@lumn             % insert in left column?
\newif\if@wid                   % flag: this is a wide insert
\newif\if@bot                   % flag: this is a bottom insert

\def\@LET{\global\let}          % we'll use this a lot

%--------------------------------------------------*
% Until you say \SetDoubleColumns, the instructions \doublecolumns,
% \enddoublecolumns, \leftcolrule and \rightcolrule and so on are 
% simply \relax.  This is so you can put these in a document which
% uses double columns, but then print it with one of the single
% column formats without them getting in the way, or vice versa.
%

\colwidth=\hsize                % default column width is \hsize

\def\doublecolumns{\relax}      \def\enddoublecolumns{\relax}
\def\leftcolrule{\relax}        \def\rightcolrule{\relax}
\def\longequation{\relax}       \def\endlongequation{\relax}
\def\wideequation{\relax}       \def\endwideequation{\relax}
\def\newcolumn{\relax}          \def\widetopinsert{\topinsert}
\def\widepageinsert{\pageinsert}\def\widebottominsert{\bottominsert}
\let\widefootnote=\footnote     \let\widevfootnote=\vfootnote

%  Save Plain definitions of inserts so we can restore them later

\let\@plaintopinsert=\topinsert  \let\@plainmidinsert=\midinsert
\let\@plainbottominsert=\bottominsert\let\@plainheavyinsert=\heavyinsert
\let\@plainpageinsert=\pageinsert\let\@plainendinsert=\endinsert
\let\@plainvfootnote=\vfootnote  \let\@plainfootnote=\footnote


% \SetDoubleColumns<column-width> sets things up for double column mode
% with columns of the given width, using the current settings for \vsize
% and \hsize.

\def\SetDoubleColumns#1{% set up double column mode
   \global\colwidth=#1\relax                    % column width
   \pagewidth=\hsize \pageheight=\vsize         % page sizes
   \@bigColHeight=\vsize                        % total height = \vsize
   \multiply \@bigColHeight by 2                % times 2
   \@leftpluscenter=\pagewidth                  % \@leftpluscenter = size
   \advance \@leftpluscenter by -\colwidth      % to right column
   \dimen\NWins=\pageheight \dimen\NEins=\pageheight % maximum top insert size
   \dimen\SWins=\pageheight \dimen\SEins=\pageheight % max bottom insert
   \output={\@nepageout{\pagecontents}}%        % new \output, single columns
   \let\doublecolumns=\@doublecolumns           % enable \doublecolumns
   \let\rightcolrule=\@rightcolrule             % enable rule
   \let\leftcolrule=\@leftcolrule               %
   \let\longequation=\@longequation             % enable wide eqns.
   \let\wideEquation=\@longequation             %
}

%  \setdoublecolumns<page-width><page-height><column-width> is included
%  for backward compatability with TeXsis 2.15 and earlier.

\def\setdoublecolumns#1#2#3{%
   \emsg{> Please use \string\SetDoubleColumns\ instead}%
   \global\hsize=#1\global\vsize=#2\relax
   \SetDoubleColumns{#3}}


%     \@doublecolumns starts double column output. It redefines \endinsert
% to handle double column insertions and \widetopinsert and \widepageinsert
% to do them.  The inserts are made global so that they get to \output
% from inside groups.

\def\@doublecolumns{% begin double column formatting
   \begingroup                                  % keep changes local
   \def\enddoublecolumns{\@enddoublecolumns}%   % enable \enddoublecolumns
   \def\doublecolumns{\relax}%                  % in case twice
   \def\endmode{\@enddoublecolumns}%            % implicit end, if needed
   \let\newcolumn=\@newcolumn                   %
%
   \output={\global\setbox\partialpage=\vbox{%  % save page so far, 
      \ifvoid\topins\else\unvbox\topins         %   including top inserts
         \bigskip\fi                            %   with some space between
         \unvbox255                             %   main page
      }}\eject                                  % in \partialpage
   \output={\@doublecolumnout}%                 % set to 2 column output
%
   \@saveVsize=\vsize                           % save old \vsize
   \hsize=\colwidth \vsize=\@bigColHeight       % set width to column width,
   \advance\vsize by -2\ht\partialpage          %   height to 2*page minus
   \advance\vsize by -2\dp\partialpage          %   what's already there
   \global\s@veskip=\spaceskip                  % save old interword glue
   \global\spaceskip=\doublecolskip             % stretch for small cols.
   \global\displaywidth=\colwidth               % equations have \colwidth
   \global\hyphenpenalty=0                      % hyphens are OK
   \multiply\vbadness by 2 \multiply\hbadness by 2 % be more tolerant
   \clubpenalty=150                             % club line penalty
   \widowpenalty=150                            % widow line penalty
% Set macros to their double column dopplegangers
   \@LET\topinsert=\@doubletopinsert
   \@LET\bottominsert=\@doublebottominsert
   \@LET\pageinsert=\@doublefullinsert
   \@LET\midinsert=\@doublemidinsert
   \@LET\heavyinsert=\@doubleheavyinsert
   \@LET\endinsert=\@enddoubleinsert     
   \@LET\widetopinsert=\@widetopinsert
   \@LET\widepageinsert=\@widepageinsert
   \@LET\widebottominsert=\@widebottominsert
   \@LET\vfootnote=\@doubleVfootnote            % \footnote uses this one
   \@LET\widefootnote=\@widefootnote    
   \@LET\widevfootnote=\@wideVfootnote
}


% \@enddoublecolumns ends double column output and balances the columns.
% This also allows for double width equations. The grouping insures that
% \endinsert is reset to the Plain version.

\def\@enddoublecolumns{% end double column mode, go back to single column
   \global\output={\@balancecolumns}\eject      % balance & output so far
   \global\output={\@nepageout{\pagecontents}}% % back to single column output
   \global\vsize=\@saveVsize                    % reset vsize
   \endgroup                                    % end 2 col. group
   \pagegoal=\vsize                             % reset overall goal size
   \spaceskip=\s@veskip                         % reset interword glue...
   \hyphenpenalty=50 \displaywidth=\hsize 
   \def\endmode{\relax}%                        % reset \endmode
% Reset macros to single column version:
   \@LET\topinsert=\@plaintopinsert
   \@LET\midinsert=\@plainmidinsert
   \@LET\pageinsert=\@plainpageinsert
   \@LET\endinsert=\@plainendinsert   
   \@LET\bottominsert=\@bottominsert
   \@LET\heavyinsert=\@heavyinsert    
   \@LET\vfootnote=\@plainvfootnote
   \@LET\widetopinsert=\@plaintopinsert
   \@LET\widepageinsert=\@plainpageinsert
   \@LET\widefootnote=\@plainfootnote
   \@LET\widebottominsert=\@plainbottominsert
   \@LET\widevfootnote=\@plainvfootnote
}% end of \@enddoublecolumns

\def\begindoublecolumns{\doublecolumns}         % synonym
\def\singlecolumn{\enddoublecolumns}            % synonym


% How to skip to a new column.  If we are in the left column, fill it
% up to force a skip to the right.  If in the right column, skip to the
% next page.

\def\@newcolumn{% skip to next column, left or right
      \vskip\z@                                 % force vertical mode
      \ifdim\pagetotal<\pageheight              % left column?
        \dimen@=\pageheight \advance\dimen@ by -\pagetotal % room left in left
        \vskip\dimen@\goodbreak                 % fill up to end of left col
      \else \vfill\eject \fi}                   % else skip to next page

%--------------------------------------------------*
% FLOATING INSERTIONS:

% Since there can now be insertions at the top and bottom of both
% the left and right columns, they will be labeled by compass points.

\newinsert\NWins \skip\NWins=0pt \newinsert\SWins \skip\SWins=0pt
\newinsert\NEins \skip\NEins=0pt \newinsert\SEins \skip\SEins=0pt


% There are also insertions for footnotes at the bottom of either column

\newinsert\LFins \count\LFins=1000 \dimen\LFins=5cm \skip\LFins=\bigskipamount 
\newinsert\RFins \count\RFins=1000 \dimen\RFins=5cm \skip\RFins=\bigskipamount


%  \@enddoubleinsert is a modified version of \endinsert which
%  decides whether to put an insertion in the left or the right column.
%  \endinsert is let equal this in \doublecolumns mode.

\def\@enddoubleinsert{% end an \insert in double column mode
   \egroup                                      % finish the \vbox\z@
%
% Decide whether in left or right column:
%
   \ifdim\pagetotal<\pageheight\leftc@lumntrue  % left if page total < 1 col
      \else \leftc@lumnfalse\fi                 %   right otherwise
   \ifx L\LRf@rce \leftc@lumntrue \fi           % or forced left
   \ifx R\LRf@rce \leftc@lumnfalse \fi          % or forced right
%
% If midinsert requested, decide whether there is room...
%
   \if@mid                                      % midinsert selected
      \dimen@=\ht\z@ \advance\dimen@ by \dp\z@  % dimen0 = height + depth
      \advance\dimen@ by \baselineskip          % + baselineskip
      \advance\dimen@ by \pagetotal             % + page total
      \ifleftc@lumn                             % if in left column
         \ifdim\dimen@>\pageheight              % \pageheight = 1 col height
         \@midfalse\p@gefalse\fi                % top insert
      \else                                     % in right column
         \ifdim\dimen@>\@bigColHeight           % \@bigColHeight = 2 col height
         \@midfalse\p@gefalse\fi\fi             % top insert
   \fi                                          % end if@mid
%
% If room for midinsert, do it; otherwise make insert in same column.
%
   \if@mid \bigskip\box\z@\bigbreak             % fits: just do it
   \else                                        % otherwise: where to put it?
      \if@wid                                   % wide insert
         \if@bot\let\@whichins=\botins          %   bottom?
         \else\let\@whichins=\topins\fi         %   or top?
      \else                                     % not wide, so...
         \if@bot                                % bottom?
            \ifleftc@lumn\let\@whichins=\SWins  %   bottom left is SW
            \else \let\@whichins=\SEins\fi      %   bottom right is SE
         \else                                  % top?
            \ifleftc@lumn\let\@whichins=\NWins  %   top left is NW
            \else \let\@whichins=\NEins\fi      %   top right is NE
         \fi                                    %
      \fi                                       % end of \if@wid
      \C@lumnInsert\@whichins                   % do the insertion
   \fi                                          % end \if@mid
   \endgroup                                    % end the insertion group
   \global\let\LRf@rce=X                        % reset forcing flag
}


% \C@lumnInsert{<insert#>} makes an appropriate insertion of the
% material into the named insert. It also inserts a \bigskip after or
% before the inserted box, just like the Plain \endinsert. Note that
% all the skips for these inserts are 0pt.

\def\C@lumnInsert#1{% make an insertion into insertion #1
   \if@wid\count#1=2000\relax                   % wide inserts count x 2
   \else\count#1=1000\fi                        % otherwise x 1
   \insert#1{%                                  % make the insertion
      \penalty100 \splitmaxdepth=\maxdimen      %   
%%    \topskip=\z@skip \splittopskip=\z@skip    %
      \floatingpenalty=\z@                      % no penalty for floating
      \if@wid\hsize=\pagewidth\fi               % full width
      \ifp@ge \dimen@=\dp\z@                    % dimen0 = depth
         \vbox to\pageheight{\unvbox\z@ \kern-\dimen@}% full page = \pageheight
      \else                                     % not full page
         \ifx#1\botins\bigskip\fi               % skip before bottom insert
         \ifx#1\SWins\bigskip\fi                % skip before bottom insert
         \ifx#1\SEins\bigskip\fi                % skip before bottom insert
         \box\z@\nobreak                        % now add box0
         \ifx#1\topins\bigskip\fi               % space below top insert
         \ifx#1\NWins\bigskip\fi                % space below top insert
         \ifx#1\NEins\bigskip\fi                % space below top insert
      \fi                                       % end of \ifp@ge
   }%                                           % end of insert
}


%     \wideXXXinsert make floating insertions across both columns. They
% use the same insert as the normal (single column) insert of the same
% name because it goes in the same place. 

\def\@widetopinsert{% make a full width (wide) insertion at top of page
   \@midfalse\p@gefalse\@widtrue\@botfalse
   \@ins \hsize=\pagewidth}   

\def\@widepageinsert{% full width, full length (i.e. full page) insertion
   \@midfalse\p@getrue\@widtrue\@botfalse       % wide page insert
   \@ins \hsize=\pagewidth}   

\def\@widebottominsert{% full width insertion at bottom of page
   \@midfalse\p@gefalse\@widtrue\@bottrue       % wide page insert
   \@ins \hsize=\pagewidth}    


%       \@doubleXXXinsert is like \XXXinsert in Plain but also sets
% \@widfalse to prevent wide inserts.

\def\@doubletopinsert{\@midfalse\p@gefalse\@botfalse\@widfalse\@ins}
\def\@doublemidinsert{\@midtrue\@botfalse\@widfalse\@ins}
\def\@doublefullinsert{\@midfalse\p@getrue\@botfalse\@widfalse\@ins}
\def\@doublebottominsert{\@midfalse\p@gefalse\@bottrue\@widfalse\@ins}
\def\@doubleheavyinsert{\@midtrue\p@gefalse\@bottrue\@widfalse\@ins}



% \forceleft and \forceright force left and right insertions independent
% of the current column position.

\def\forceleft{\global\let\LRf@rce=L}           % force left insert
\def\forceright{\global\let\LRf@rce=R}          % force right insert

\let\LRf@rce=X                                  % default is no force

%--------------------------------------------------*
% FOOTNOTES:  wide footnotes go across the bottom of both columns,
% while the others just go in the left or right column.  The names
% begin with @ because these are only enabled in double column mode.

\def\@widefootnote#1{% footnote across a double column page
  \let\@sf=\empty % parameter #2 (the text) is read later
  \ifhmode\edef\@sf{\spacefactor\the\spacefactor}\/\fi
  #1\@sf\@wideVfootnote{#1}}

\def\@wideVfootnote#1{\insert\footins\bgroup
  \hsize=\pagewidth                             % as wide as a page
  \interlinepenalty=\interfootnotelinepenalty
  \splittopskip=\ht\strutbox % top baseline for broken footnotes
  \splitmaxdepth=\dp\strutbox \floatingpenalty=\@MM
  \leftskip=\z@skip \rightskip=\z@skip \spaceskip=\z@skip \xspaceskip=\z@skip
  \textindent{#1}\footstrut\futurelet\next\fo@t}

\def\@doubleVfootnote#1{% double column footnote in left or right column
   \ifdim\pagetotal<\pageheight\relax   %
        \def\next{\@dblVfootnote\LFins{#1}}%
   \else\def\next{\@dblVfootnote\RFins{#1}}%
   \fi\next}

\def\@dblVfootnote#1#2{% footnote insert in whichever column named by #1
   \insert#1\bgroup                             % begin insert
     \interlinepenalty\interfootnotelinepenalty %
     \splittopskip=\ht\strutbox % top baseline for broken footnotes
     \splitmaxdepth=\dp\strutbox \floatingpenalty\@MM %
     \leftskip=\z@skip \rightskip=\z@skip      %
     \spaceskip=\z@skip \xspaceskip=\z@skip    %
     \textindent{#2}\footstrut\futurelet\next\fo@t}

%
%--------------------------------------------------*
% OUTPUT ROUTINES for double columns:


% \@nepageout ships out a single page with running headlines
% and footlines added.  Can be used with single or double columns,
% depending on what you put as the argument.

\def\@nepageout#1{%                             % output one page
   \shipout\vbox{%                              % output a box
      \offinterlineskip                         % no interline spacing!
      \wideheadline                             % make wide headline
      \vbox to \pageheight{\boxmaxdepth=\maxdepth %
          #1\relax}%                            % box containing #1
      \widefootline}%                           % make wide footline
   \advancepageno}%                             % increment page number


% The following are like \makeheadline and \makefootline in Plain
% except that they use \hbox to\pagewidth instead of \line.  

\def\wideheadline{% \makeheadline for double column mode
   \vbox to\z@{\vskip-22.5\p@                   % skip up some
      \ifx\undefined\headlineoffset\else\vskip-\headlineoffset\fi
      \hbox to \pagewidth{\vbox to 8.5\p@{}\the\headline}% content in \headline
      \vss}%            
   \nointerlineskip}%   

\def\widefootline{% \makefootline for double column mode
   \baselineskip=24\p@                          % space down
      \ifx\undefined\footlineoffset\else\vskip\footlineoffset\fi
   \hbox to \pagewidth{\the\footline}}%         % content in \footline


% \@doublecolumnout splits the page into two columns, including any
% insertions which have accumulated.

\def\@doublecolumnout{% output routine for double column mode
%   
% get height of columns in \dimen@
%
   \dimen@=\pageheight                          % start with total space
   \advance\dimen@ by -\ht\partialpage          % subtract used height
   \advance\dimen@ by -\dp\partialpage          % ... and deptn
   \ifvoid\topins\else                          % subtract top inserts
      \advance\dimen@ by -\ht\topins            %
      \advance\dimen@ by -\dp\topins            %
      \advance\dimen@ by -\bigskipamount        % including skip
      \advance\dimen@ by -\splittopskip\fi      % and extra at top of cols.
   \ifvoid\botins\else                          % subtract any bottom inserts
      \advance\dimen@ by -\ht\botins            %
      \advance\dimen@ by -\dp\botins            %
      \advance\dimen@ by -\bigskipamount\fi     % including skip
   \ifvoid\footins\else                         % subtract full width footnotes
      \advance\dimen@ by -\ht\footins           %
      \advance\dimen@ by -\dp\footins           %
      \advance\dimen@ by -\skip\footins\fi      % including skip
   \@saveSplitmax=\splitmaxdepth \splitmaxdepth=\colmaxdepth 
   \splittopskip=\topskip
%
% construct left and right columns, with inserts inserted, and force
% them to the desired size \dimen@
%
   \ifdim\dimen@>\baselineskip                  % if room for at least 1 line
      \MakeColumn{1}{255}{\dimen@}{\NWins}{\LFins}{\SWins}%
      \MakeColumn{2}{255}{\dimen@}{\NEins}{\RFins}{\SEins}%
      \setbox1=\vbox to \dimen@{\unvbox1}%      % reset to same size
      \setbox2=\vbox to \dimen@{\unvbox2}%      % reset to same size 
   \else                                        % ... else no room
      \setbox1=\vbox{}\setbox2=\vbox{}%         % so just empty columns
   \fi                                          % end if room for columns
%
   \@nepageout{\@pagesofar\@pagebottom}%        % ship out double column page
   \global\vsize=\@bigColHeight                 %
   \unvbox255 \penalty\outputpenalty            % put remaining text back
   \splitmaxdepth=\@saveSplitmax}               % reset \splitmaxdepth


% \MakeColumn{outbox}{inbox}{size}{topinsert}{footinsert}{bottominsert}
% creates a column of text of the given length, with the topinsert added
% at the top, and the footnote and bottominsert added at the bottom
% of the column (in that order).  The result is put in outbox, while
% what is left over remains in inbox.  

\def\MakeColumn#1#2#3#4#5#6{% make a column with top and bottom inserts
%
% start the column with the topinsert (#4) and the main text (#2)
%
   \setbox3=\vbox{\ifvoid#4\else\unvbox#4\vskip\skip#4\fi \unvbox#2}%
%
% also collect column footnotes (#5) and bottom inserts (#6)
%

   \setbox4=\vbox{\ifvoid#5\else\vskip\skip#5\footnoterule\unvbox#5\fi%
       \ifvoid#6\else\vskip\skip#6\unvbox#6\fi}% 
% 
% split off just right amount from top stuff to make output column
%
   \dimen@ii=#3\relax
   \advance\dimen@ii by -\ht4 \advance\dimen@ii by -\dp4\relax
   \setbox#1=\vsplit3 to \dimen@ii 
%
% put the top and bottom together; put remainder from split back in input
%
   \setbox#1=\vbox{\unvbox#1\unvbox4}%
   \setbox#2=\vbox{\unvbox3}%
}


% \@pagesofar adds double column material to the page.  The left column
% is in box 1, and the right column is in box 2

\def\@pagesofar{% add stuff to top of page collected so far
   \ifvoid\topins\else\unvbox\topins            % wide top inserts, if any?
       \vskip\skip\topins\fi                    % some space below them
   \unvbox\partialpage                          % partial page from past?
   \wd1=\hsize \wd2=\hsize                      % set column sizes
   \hbox to \pagewidth{\box1\hfill\box2}}%      % combine 2 column boxes


% \@pagebottom puts the (wide) bottom and footnote inserts in place,
% if there are any.

\def\@pagebottom{% add inserts to bottom of a page
   \ifvoid\botins\else\bigskip\unvbox\botins\fi % wide bottom inserts, if any
   \ifvoid\footins\else                         % wide footnotes, if any
      \vskip\skip\footins\footnoterule          % skip and rule above them
      \unvbox\footins\fi}                       % then the footnotes


% \@balancecolumns is the output routine for balancing 2 columns. 
% (Based loosely on \balancecolumns from The TeXbook, pg 417)
   
\def\@balancecolumns{% balance partial double columns page
%
% get target column height from sum of text and all inserts 
%
   \setbox255=\vbox{\unvbox255}% reset glue
   \dimen@=\ht255 \advance\dimen@ by \dp255     % main text  
   \@addsize\dimen@\NWins \@addsize\dimen@\NEins % top inserts
   \@addsize\dimen@\LFins \@addsize\dimen@\RFins % column footnotes
   \@addsize\dimen@\SWins \@addsize\dimen@\SEins % bottom inserts
   \divide \dimen@ by 2                         % and divide by 2
   \@saveSplitmax=\splitmaxdepth                %
   \splitmaxdepth=\colmaxdepth                  %
   \splittopskip=\topskip                       % top skip for splits
%
% Loop over possible splits of text into left and right columns.
% Always use copies of boxes to avoid destroying contents.
%
   \advance\dimen@ by -.5\baselineskip          % and a smidgeon LESS
   {\vbadness=20000 \loop                       % suppress errors
      \setbox0=\copy255                         %
      \setbox5=\copy\NWins \setbox6=\copy\LFins\setbox7=\copy\SWins
      \setbox8=\copy\NEins \setbox9=\copy\RFins \setbox10=\copy\SEins
      \MakeColumn{1}{0}{\dimen@}{5}{6}{7}%      % first column fixed height
      \MakeColumn{2}{0}{\pageheight}{8}{9}{10}% % second big enuf for all
      \ifdim\ht2>\ht1
        \global\advance\dimen@ by 1pt 
      \repeat}%                                 %   increment and try again
%
% End loop over possible splits.
%
   \MakeColumn{1}{255}{\dimen@}{\NWins}{\LFins}{\SWins}%
   \MakeColumn{2}{255}{\pageheight}{\NEins}{\RFins}{\SEins}%
   \dimen@=\ht1 \ifdim\ht2>\ht1 \dimen@=\ht2 \fi % larger of two
   \setbox1=\vbox to \dimen@{\unvbox1}%         % reset to same size
   \setbox2=\vbox to \dimen@{\unvbox2}%         % reset to same size 
   \splitmaxdepth=\@saveSplitmax                % restore \splitmaxdepth
   \output={\@balancingerror}%                  % prepare for error
   \@pagesofar}                                 % put columns on page


\def\@addsize#1#2{% add size of box/insert #2 to counter #1 
   \ifvoid#2\else\advance#1 by \skip#2\relax    % unless void, add skip,
     \advance#1 by \ht#2 \advance#1 by \dp#2\relax % and height and depth
   \fi}


% If the balanced columns fill the page then \output will be called
% again, and this error message will be displayed.

\newhelp\@balncErrormsg{%
@balancecolumns: I couldn't figure out how to balance the^^M
two columns.  Maybe you can re-arange some text to make ^^M
the job easier.  Try typing i\string\vfill to see the page anyway.}

\def\@balancingerror{% error, columns not balanced before page finished
   \newlinechar=`\^^M                           % ^^M is line break
   \errhelp=\@balncErrormsg                     % longer help message
   \errmessage{Page cannot be balanced}%        % error message
   \@nepageout{\unvbox255}}%                    % do something anyway


%--------------------------------------------------*
% \@leftcolrule and \@rightcolrule put rules across left and right
% columns for spanned equations

\def\@leftcolrule{%     Rule across bottom of left column
   \vskip 2pt\nointerlineskip   % some whitespace first
   \hbox to \pagewidth{%                % left column
       \vbox to 6pt{\vfil \hrule width\colwidth height\rulewd}%
       \hbox{\vrule height 6pt width\rulewd}\hfill}%
   \smallskip\nobreak}

\def\@rightcolrule{% rule across top of a right column after balancing
   \vskip\baselineskip\nointerlineskip
   \hbox to \pagewidth{\hfill   % stretch across to right column
       \hbox{\vrule height 6pt width\rulewd}%
       \vbox to 6pt{\hrule width\colwidth height\rulewd \vfil}}%
   \vskip 2pt}

\def\@longequation{%
   \enddoublecolumns            % balance what we have
   \@leftcolrule                % rule below to separage
   \def\endlongequation{\@endlongequation}} % enable

\def\@endlongequation{%
    \@rightcolrule              % with the rule at top of right column
    \doublecolumns}             % then back to double column mode
                                                
                                                

\def\longequation{\relax}                       % default for single column
\def\endlongequation{\relax}                    %   does nothing

%------------------------*
% Plain.tex compatibility:
% If these macros are called from plain TeX \botins won't be defined, so
% just fake it. 

\ifx\undefined\botins \let\botins=\topins \fi

% These definitions are copied from TXSinit.tex so that TXSdcol.tex
% can be used with Plain and bottom inserts in columns will work. The
% \if@bot is just ignored by the Plain \endinsert.

\def\topinsert{\@midfalse\p@gefalse\@botfalse\@ins}
\def\midinsert{\@midtrue\p@gefalse\@botfalse\@ins}
\def\pageinsert{\@midfalse\p@getrue\@botfalse\@ins}
\def\bottominsert{\@midfalse\p@gefalse\@bottrue\@ins}
\def\heavyinsert{\@midtrue\p@gefalse\@bottrue\@ins}

\def\pagecontents{%  constructs page contents, including bottom inserts
   \ifvoid\topins\else\unvbox\topins    % top inserts, if any
      \vskip\skip\topins\fi             % and some space below
   \dimen@=\dp\@cclv \unvbox\@cclv      % main page contents from \box255
   \ifvoid\botins\else\bigskip          % bottom inserts? space above
      \unvbox\botins\fi                 % and then insert the text
   \ifvoid\footins\else                 % footnote inserts, if present
      \vskip\skip\footins               % skip above
      \footnoterule                     % put the rule above footnotes
      \unvbox\footins\fi                % then the footnotes
   \ifr@ggedbottom \kern-\dimen@ \vfil \fi}

\catcode`@=12                   % @ back to a letter
% >>> EOF TXSdcol.tex <<<

